Characterization of MKIDs for CMB observation at 220 GHz with the South Pole Telescope

We present an updated design of the 220 GHz microwave kinetic inductance detector (MKID) pixel for SPT-3G+, the next-generation camera for the South Pole Telescope. We show results of the dark testing of a 63-pixel array with mean inductor quality factor $Q_i = 4.8 \times 10^5$, aluminum inductor transition temperature $T_c = 1.19$ K, and kinetic inductance fraction $\alpha_k = 0.32$. We optically characterize both the microstrip-coupled and CPW-coupled resonators, and find both have a spectral response close to prediction with an optical efficiency of $\eta \sim 70\%$. However, we find slightly lower optical response on the lower edge of the band than predicted, with neighboring dark detectors showing more response in this region, though at level consistent with less than 5\% frequency shift relative to the optical detectors. The detectors show polarized response consistent with expectations, with a cross-polar response of $\sim 10\%$ for both detector orientations.

==> authors.tex <==


%Authors

\author{
K.~R.~Dibert\textsuperscript{1,2},
P.~S.~Barry\textsuperscript{3,4},
A.~J.~Anderson\textsuperscript{1,2,5},
B.~A.~Benson\textsuperscript{1,2,5},
T.~Cecil\textsuperscript{4},
C.~L.~Chang\textsuperscript{1,2,4},
K.~N.~Fichman\textsuperscript{1,2}, 
K.~Karkare\textsuperscript{1,2},
J.~Li\textsuperscript{4},
T.~Natoli\textsuperscript{1,2}, 
Z.~Pan\textsuperscript{4},
M.~Rouble\textsuperscript{6},
E.~Shirokoff\textsuperscript{1,2},
and~M.~Young\textsuperscript{2,5},

\textit{on behalf of the South Pole Telescope collaboration}


% Affiliations

\institute{
\textsuperscript{1}{Dept. of Astronomy \& Astrophysics, U. Chicago, 5640 South Ellis Avenue, Chicago, IL, 60637, USA} \\
\textsuperscript{2}{Kavli Institute for Cosmological Physics, U. Chicago, 5640 South Ellis Avenue, Chicago, IL, 60637, USA} \\
\textsuperscript{3}{School of Physics and Astronomy, Cardiff University, Cardiff CF24 3AA, UK} \\
\textsuperscript{4}{Argonne National Laboratory, 9700 South Cass Avenue., Argonne, IL, 60439, USA} \\
\textsuperscript{5}{Fermi National Accelerator Laboratory, MS209, P.O. Box 500, Batavia, IL, 60510, USA} \\
\textsuperscript{6}{Department of Physics, McGill University, 3600 Rue University, Montreal, Quebec H3A 2T8, Canada} \\
}
\vspace{-25pt}
}
